Optimizing Error-Bounded Lossy Compression for Scientific Data on GPUs

Error-bounded lossy compression is a critical technique for significantly reducing scientific data volumes. With ever-emerging heterogeneous high-performance computing (HPC) architecture, GPU-accelerated error-bounded compressors (such as cuSZ+ and cuZFP) have been developed. However, they suffer from either low performance or low compression ratios. To this end, we propose cuSZ+ to target both high compression ratios and throughputs. We identify that data sparsity and data smoothness are key factors for high compression throughputs. Our key contributions in this work are fourfold: (1) We propose an efficient compression workflow to adaptively perform run-length encoding and/or variable-length encoding. (2) We derive Lorenzo reconstruction in decompression as multidimensional partial-sum computation and propose a fine-grained Lorenzo reconstruction algorithm for GPU architectures. (3) We carefully optimize each of cuSZ+ kernels by leveraging state-of-the-art CUDA parallel primitives. (4) We evaluate cuSZ+ using seven real-world HPC application datasets on V100 and A100 GPUs. Experiments show cuSZ+ improves the compression throughputs and ratios by up to 18.4X and 5.3X, respectively, over cuSZ on the tested datasets.

==> eval/content_zip.tex <==
\begin{tabular}{ @{} r *{11}{ r@{} } }
                                       & \EVALTITLE{          }                                & \EVALTITLE{gather}                                       & \EVALTITLE{         }                                 & \EVALTITLE{Huffman}                                  & \EVALTITLE{zip:}                                         & \EVALTITLE{Huffman}                                  & \EVALTITLE{scatter}                                      & \EVALTITLE{       }                                   & \EVALTITLE{unzip:}                                   \\[-.6ex]& \EVALTITLE{dual-quant} & \EVALTITLE{outlier} & \EVALTITLE{histogram} & \EVALTITLE{encoding} & \EVALTITLE{all kernels} & \EVALTITLE{decoding} & \EVALTITLE{outlier} & \EVALTITLE{reconst} & \EVALTITLE{all kernels}  \\
    \raisebox{1.5pt}{\scriptsize 8280} & \BARdefault{589.7}{1.00}{6.379629813681621}{gray!40}  & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} &                                                       & \BARdefault{400.0}{1.00}{5.991464547107982}{gray!40} & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{196.0}{1.00}{5.278114659230517}{gray!40} & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{300.0}{1.00}{5.703782474656201}{gray!40}  & \BARdefault{118.5}{1.00}{7.162981810742686}{gray!40} \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 7742} & \BARdefault{775.5}{1.32}{8.389971824618101}{black}    & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} &                                                       & \BARdefault{400.0}{1.00}{5.991464547107982}{black}   & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{196.0}{1.00}{5.278114659230517}{black}   & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{300.0}{1.00}{5.703782474656201}{black}    & \BARdefault{118.5}{1.00}{7.162981810742686}{black}   \\[-1.0ex]
    \\[-1ex]
    \raisebox{1.5pt}{\scriptsize 8280} & \BARdefault{531.6}{1.00}{6.275884784638269}{gray!40}  & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} &                                                       & \BARdefault{400.0}{1.00}{5.991464547107982}{gray!40} & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{502.2}{1.00}{6.218998446723485}{gray!40} & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{300.0}{1.00}{5.703782474656201}{gray!40}  & \BARdefault{187.8}{1.00}{7.8531344520656}{gray!40}   \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 7742} & \BARdefault{551.8}{1.04}{6.5140321983410585}{black}   & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} &                                                       & \BARdefault{400.0}{1.00}{5.991464547107982}{black}   & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{502.2}{1.00}{6.218998446723485}{black}   & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{300.0}{1.00}{5.703782474656201}{black}    & \BARdefault{187.8}{1.00}{7.8531344520656}{black}     \\[-1.0ex]
    \\[-1ex]
    \raisebox{1.5pt}{\scriptsize 8280} & \BARdefault{392.8}{1.00}{5.973254352550253}{gray!40}  & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} &                                                       & \BARdefault{400.0}{1.00}{5.991464547107982}{gray!40} & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{524.5}{1.00}{6.262445427836352}{gray!40} & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{300.0}{1.00}{5.703782474656201}{gray!40}  & \BARdefault{190.8}{1.00}{7.877176140739349}{gray!40} \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 7742} & \BARdefault{443.4}{1.13}{6.742473997206886}{black}    & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} &                                                       & \BARdefault{400.0}{1.00}{5.991464547107982}{black}   & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{524.5}{1.00}{6.262445427836352}{black}   & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{300.0}{1.00}{5.703782474656201}{black}    & \BARdefault{190.8}{1.00}{7.877176140739349}{black}   \\[-1.0ex]
    \\[-1ex]
    \raisebox{1.5pt}{\scriptsize 8280} & \BARdefault{362.6}{1.00}{5.8933883100061655}{gray!40} & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} &                                                       & \BARdefault{400.0}{1.00}{5.991464547107982}{gray!40} & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{670.4}{1.00}{6.507874549167873}{gray!40} & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{300.0}{1.00}{5.703782474656201}{gray!40}  & \BARdefault{207.3}{1.00}{8.000922999291351}{gray!40} \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 7742} & \BARdefault{417.9}{1.15}{6.7914421767039705}{black}   & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} &                                                       & \BARdefault{400.0}{1.00}{5.991464547107982}{black}   & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{670.4}{1.00}{6.507874549167873}{black}   & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{300.0}{1.00}{5.703782474656201}{black}    & \BARdefault{207.3}{1.00}{8.000922999291351}{black}   \\[-1.0ex]
    \\[-1ex]
    \raisebox{1.5pt}{\scriptsize 8280} & \BARdefault{378.0}{1.00}{5.934967919057073}{gray!40}  & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} &                                                       & \BARdefault{400.0}{1.00}{5.991464547107982}{gray!40} & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{660.3}{1.00}{6.492694277200526}{gray!40} & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{300.0}{1.00}{5.703782474656201}{gray!40}  & \BARdefault{206.3}{1.00}{7.993846524319199}{gray!40} \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 7742} & \BARdefault{407.9}{1.08}{6.403825152779289}{black}    & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} &                                                       & \BARdefault{400.0}{1.00}{5.991464547107982}{black}   & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{660.3}{1.00}{6.492694277200526}{black}   & \scriptsize\color{gray}\raisebox{1.5pt}{n/a}\hspace{2em} & \BARdefault{300.0}{1.00}{5.703782474656201}{black}    & \BARdefault{206.3}{1.00}{7.993846524319199}{black}   \\[-1.0ex]
    \\[-1ex]
    \raisebox{1.5pt}{\scriptsize A100} & \BARdefault{506.4}{1.54}{8.937085136553828}{Bv}       & \BARdefault{266.8}{1.21}{6.507703813791978}{Bv}          & \BARdefault{828.4}{1.46}{9.278426336274007}{Bv}       & \BARdefault{135.3}{2.32}{9.432680623585446}{Bv}      & \BARdefault{66.7}{1.79}{6.470656098035423}{Bv}           & \BARdefault{40.3}{0.96}{3.581234163656426}{Bv}       & \BARdefault{535.9}{2.38}{12.899374042669244}{Bv}         & \BARdefault{485.9}{1.57}{9.021968903141461}{Bv}       & \BARdefault{34.8}{1.09}{5.67828964159803}{Bv}        \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize V100} & \BARreference{328.3}{1.00}{5.793927824507547}{Y}      & \BARreference{221.4}{1.00}{5.399831188462675}{Y}         & \BARreference{565.9}{1.00}{6.338412409036244}{Y}      & \BARreference{58.3}{1.00}{4.065774852546369}{Y}      & \BARreference{37.3}{1.00}{3.6196822919692626}{Y}         & \BARreference{42.1}{1.00}{3.7396913428348797}{Y}     & \BARreference{225.0}{1.00}{5.416066173818256}{Y}         & \BARreference{308.7}{1.00}{5.732432644035251}{Y}      & \BARreference{31.8}{1.00}{5.189262415253699}{Y}      \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 3080} & \BARpattern{160.4}{0.49}{2.830317781420793}{Bv!60}    & \BARpattern{124.7}{0.56}{3.042719726719831}{Bv!60}       & \BARpattern{694.5}{1.23}{7.77878898607379}{Bv!60}     & \BARpattern{83.0}{1.42}{5.785875263289055}{Bv!60}    & \BARpattern{36.0}{0.97}{3.4954533198145805}{Bv!60}       & \BARpattern{51.2}{1.22}{4.5535433701697725}{Bv!60}   & \BARpattern{428.8}{1.91}{10.322995746675467}{Bv!60}      & \BARpattern{262.5}{0.85}{4.873540506357448}{Bv!60}    & \BARpattern{39.0}{1.23}{6.360078984452499}{Bv!60}    \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 8000} & \BARpattern{117.6}{0.36}{2.0747372351417432}{gray!20} & \BARpattern{134.3}{0.61}{3.275508388727654}{gray!20}     & \BARpattern{348.3}{0.62}{3.901171485988176}{gray!20}  & \BARpattern{49.5}{0.85}{3.4485946571315718}{gray!20} & \BARpattern{25.6}{0.69}{2.4837942520103313}{gray!20}     & \BARpattern{32.9}{0.78}{2.926671994113881}{gray!20}  & \BARpattern{135.5}{0.60}{3.262287120438009}{gray!20}     & \BARpattern{188.5}{0.61}{3.4999439828981895}{gray!20} & \BARpattern{23.2}{0.73}{3.790719915960578}{gray!20}  \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 5000} & \BARpattern{92.0}{0.28}{1.6240402051358027}{gray!10}  & \BARpattern{90.3}{0.41}{2.201799543753061}{gray!10}      & \BARpattern{225.9}{0.40}{2.529837052267538}{gray!10}  & \BARpattern{46.4}{0.80}{3.2370183544484687}{gray!10} & \BARpattern{20.9}{0.56}{2.0239776568800063}{gray!10}     & \BARpattern{24.4}{0.58}{2.166014331820022}{gray!10}  & \BARpattern{181.2}{0.81}{4.361632060839552}{gray!10}     & \BARpattern{143.8}{0.47}{2.6695953495298794}{gray!10} & \BARpattern{18.7}{0.59}{3.0500769972217707}{gray!10} \\[-1.0ex]
    \\[-1ex]
    \raisebox{1.5pt}{\scriptsize A100} & \BARdefault{382.8}{1.40}{7.844343576472383}{Bv}       & \BARdefault{105.3}{0.66}{3.3321353143282035}{Bv}         & \BARdefault{256.2}{0.72}{4.222988578092379}{Bv}       & \BARdefault{115.6}{1.07}{5.022801724265289}{Bv}      & \BARdefault{39.3}{0.88}{3.336231381502176}{Bv}           & \BARdefault{46.4}{1.22}{4.4497924609205155}{Bv}      & \BARdefault{478.9}{1.43}{8.31498220932123}{Bv}           & \BARdefault{410.9}{1.54}{8.599288750260945}{Bv}       & \BARdefault{38.3}{1.27}{6.491856260926021}{Bv}       \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize V100} & \BARreference{273.9}{1.00}{5.612763076269032}{Y}      & \BARreference{160.6}{1.00}{5.078655438586857}{Y}         & \BARreference{356.5}{1.00}{5.876209288643253}{Y}      & \BARreference{107.7}{1.00}{4.679330593470557}{Y}     & \BARreference{44.8}{1.00}{3.8023761850758246}{Y}         & \BARreference{37.9}{1.00}{3.634344712779796}{Y}      & \BARreference{334.8}{1.00}{5.813518614219366}{Y}         & \BARreference{267.0}{1.00}{5.587079685908097}{Y}      & \BARreference{30.2}{1.00}{5.1107892800725665}{Y}     \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 3080} & \BARpattern{153.0}{0.56}{3.1353627980954806}{Bv!60}   & \BARpattern{202.8}{1.26}{6.414374757529681}{Bv!60}       & \BARpattern{420.1}{1.18}{6.92529266115317}{Bv!60}     & \BARpattern{101.8}{0.95}{4.422781919907079}{Bv!60}   & \BARpattern{42.2}{0.94}{3.58493584217249}{Bv!60}         & \BARpattern{49.1}{1.30}{4.712682229536931}{Bv!60}    & \BARpattern{469.9}{1.40}{8.159396099621548}{Bv!60}       & \BARpattern{244.9}{0.92}{5.125065538336995}{Bv!60}    & \BARpattern{37.6}{1.25}{6.372924747975981}{Bv!60}    \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 8000} & \BARpattern{118.3}{0.43}{2.4242161957147372}{gray!20} & \BARpattern{114.4}{0.71}{3.6192207558392853}{gray!20}    & \BARpattern{255.9}{0.72}{4.218938844836147}{gray!20}  & \BARpattern{71.3}{0.66}{3.100056017487584}{gray!20}  & \BARpattern{28.5}{0.64}{2.41658887637301}{gray!20}       & \BARpattern{36.1}{0.95}{3.459597577349464}{gray!20}  & \BARpattern{204.3}{0.61}{3.5483342860923273}{gray!20}    & \BARpattern{168.5}{0.63}{3.525889940224453}{gray!20}  & \BARpattern{25.9}{0.86}{4.391148449465106}{gray!20}  \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 5000} & \BARpattern{92.1}{0.34}{1.8868993285122593}{gray!10}  & \BARpattern{119.1}{0.74}{3.767741804688289}{gray!10}     & \BARpattern{214.8}{0.60}{3.54099397684348}{gray!10}   & \BARpattern{53.6}{0.50}{2.326722002278049}{gray!10}  & \BARpattern{23.5}{0.52}{1.9927390572573496}{gray!10}     & \BARpattern{26.6}{0.70}{2.555637173161242}{gray!10}  & \BARpattern{266.0}{0.79}{4.618659441016914}{gray!10}     & \BARpattern{136.9}{0.51}{2.8648174974883}{gray!10}    & \BARpattern{20.6}{0.68}{3.483670012875888}{gray!10}  \\[-1.0ex]
    \\[-1ex]
    \raisebox{1.5pt}{\scriptsize A100} & \BARdefault{203.5}{1.02}{5.412430567806264}{Bv}       & \BARdefault{220.0}{0.88}{4.840697191109311}{Bv}          & \BARdefault{544.1}{1.24}{7.5495496237089705}{Bv}      & \BARdefault{140.6}{1.26}{5.954112192225575}{Bv}      & \BARdefault{54.3}{1.10}{4.293317373281949}{Bv}           & \BARdefault{40.5}{0.88}{3.382394837539056}{Bv}       & \BARdefault{758.7}{1.21}{7.782891594715541}{Bv}          & \BARdefault{222.8}{1.11}{5.898672291615282}{Bv}       & \BARdefault{32.8}{0.93}{4.978249055513834}{Bv}       \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize V100} & \BARreference{199.0}{1.00}{5.293491366770457}{Y}      & \BARreference{251.1}{1.00}{5.526041586882066}{Y}         & \BARreference{438.4}{1.00}{6.083168070230605}{Y}      & \BARreference{111.2}{1.00}{4.7115516557544215}{Y}    & \BARreference{49.3}{1.00}{3.898235360125081}{Y}          & \BARreference{45.8}{1.00}{3.8243659271413706}{Y}     & \BARreference{628.1}{1.00}{6.442626299965117}{Y}         & \BARreference{200.1}{1.00}{5.298872188202966}{Y}      & \BARreference{35.2}{1.00}{5.340902424648424}{Y}      \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 3080} & \BARpattern{149.4}{0.75}{3.9739456370101167}{Bv!60}   & \BARpattern{205.7}{0.82}{4.524949704975345}{Bv!60}       & \BARpattern{590.5}{1.35}{8.193599850304617}{Bv!60}    & \BARpattern{103.8}{0.93}{4.398471134697602}{Bv!60}   & \BARpattern{43.7}{0.89}{3.4549605017902127}{Bv!60}       & \BARpattern{54.1}{1.18}{4.514623197952262}{Bv!60}    & \BARpattern{547.6}{0.87}{5.617074959242522}{Bv!60}       & \BARpattern{231.3}{1.16}{6.124564490067836}{Bv!60}    & \BARpattern{40.6}{1.15}{6.159616687301522}{Bv!60}    \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 8000} & \BARpattern{82.6}{0.41}{2.1965049750531143}{gray!20}  & \BARpattern{135.4}{0.54}{2.9790031728085964}{gray!20}    & \BARpattern{263.8}{0.60}{3.6598589857711805}{gray!20} & \BARpattern{74.3}{0.67}{3.148201845815783}{gray!20}  & \BARpattern{27.2}{0.55}{2.1514733172476763}{gray!20}     & \BARpattern{39.5}{0.86}{3.301447462909373}{gray!20}  & \BARpattern{320.2}{0.51}{3.2851160059107456}{gray!20}    & \BARpattern{153.1}{0.77}{4.054216562038105}{gray!20}  & \BARpattern{28.6}{0.81}{4.343990535727641}{gray!20}  \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 5000} & \BARpattern{71.6}{0.36}{1.9038883104325985}{gray!10}  & \BARpattern{111.2}{0.44}{2.446108172604773}{gray!10}     & \BARpattern{201.4}{0.46}{2.7949447549765214}{gray!10} & \BARpattern{72.6}{0.65}{3.0767810393681705}{gray!10} & \BARpattern{24.0}{0.49}{1.895772661752106}{gray!10}      & \BARpattern{31.7}{0.69}{2.6481834605306114}{gray!10} & \BARpattern{275.3}{0.44}{2.824513289881466}{gray!10}     & \BARpattern{126.1}{0.63}{3.339532287471528}{gray!10}  & \BARpattern{23.2}{0.66}{3.522806891063706}{gray!10}  \\[-1.0ex]
    \\[-1ex]
    \raisebox{1.5pt}{\scriptsize A100} & \BARdefault{235.4}{1.08}{5.808159433889814}{Bv}       & \BARdefault{269.6}{1.20}{6.481238631166732}{Bv}          & \BARdefault{778.8}{1.79}{10.877606793693301}{Bv}      & \BARdefault{175.5}{1.75}{8.077610936617964}{Bv}      & \BARdefault{66.9}{1.43}{5.489757259004985}{Bv}           & \BARdefault{77.4}{1.32}{5.374884889427779}{Bv}       & \BARdefault{651.9}{2.15}{12.301059197000843}{Bv}         & \BARdefault{232.9}{1.11}{5.915784686104234}{Bv}       & \BARdefault{53.4}{1.34}{7.401956725416083}{Bv}       \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize V100} & \BARreference{218.3}{1.00}{5.3858036926717885}{Y}     & \BARreference{225.3}{1.00}{5.417589084742611}{Y}         & \BARreference{435.0}{1.00}{6.075331926188158}{Y}      & \BARreference{100.1}{1.00}{4.606168884521496}{Y}     & \BARreference{46.9}{1.00}{3.8486778053900648}{Y}         & \BARreference{58.7}{1.00}{4.071903418872878}{Y}      & \BARreference{302.8}{1.00}{5.712962885973495}{Y}         & \BARreference{210.6}{1.00}{5.349915970695764}{Y}      & \BARreference{39.8}{1.00}{5.527550129393346}{Y}      \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 3080} & \BARpattern{154.3}{0.71}{3.807454059535336}{Bv!60}    & \BARpattern{155.6}{0.69}{3.7411030100963405}{Bv!60}      & \BARpattern{684.4}{1.57}{9.55868217370885}{Bv!60}     & \BARpattern{100.5}{1.00}{4.626439972167356}{Bv!60}   & \BARpattern{41.1}{0.88}{3.3728172097996527}{Bv!60}       & \BARpattern{96.8}{1.65}{6.7153999764489365}{Bv!60}   & \BARpattern{560.0}{1.85}{10.565846011470652}{Bv!60}      & \BARpattern{243.3}{1.16}{6.181328058199509}{Bv!60}    & \BARpattern{61.6}{1.55}{8.546709904057325}{Bv!60}    \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 8000} & \BARpattern{87.3}{0.40}{2.1549957545306193}{gray!20}  & \BARpattern{140.1}{0.62}{3.368921996037918}{gray!20}     & \BARpattern{238.3}{0.55}{3.327610548129507}{gray!20}  & \BARpattern{68.5}{0.68}{3.1503497794419255}{gray!20} & \BARpattern{26.7}{0.57}{2.1933212010012837}{gray!20}     & \BARpattern{73.5}{1.25}{5.101037269081156}{gray!20}  & \BARpattern{171.9}{0.57}{3.2441681801822186}{gray!20}    & \BARpattern{153.8}{0.73}{3.906217524762164}{gray!20}  & \BARpattern{38.6}{0.97}{5.350659638876127}{gray!20}  \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 5000} & \BARpattern{78.5}{0.36}{1.9373652363603107}{gray!10}  & \BARpattern{94.5}{0.42}{2.2721315609838912}{gray!10}     & \BARpattern{177.2}{0.41}{2.47444447988324}{gray!10}   & \BARpattern{61.8}{0.62}{2.8423564471487786}{gray!10} & \BARpattern{22.1}{0.47}{1.8163107775563385}{gray!10}     & \BARpattern{68.1}{1.16}{4.725267787450514}{gray!10}  & \BARpattern{217.8}{0.72}{4.109338194435417}{gray!10}     & \BARpattern{121.6}{0.58}{3.089476304441782}{gray!10}  & \BARpattern{36.4}{0.91}{5.043904159710655}{gray!10}  \\[-1.0ex]
    \\[-1ex]
    \raisebox{1.5pt}{\scriptsize A100} & \BARdefault{205.6}{1.04}{5.5026596104050345}{Bv}      & \BARdefault{286.6}{1.23}{6.703490567063662}{Bv}          & \BARdefault{816.6}{1.47}{9.28504549469087}{Bv}        & \BARdefault{156.2}{1.70}{7.6746314590226214}{Bv}     & \BARdefault{62.6}{1.38}{5.257863549013831}{Bv}           & \BARdefault{42.3}{0.92}{3.5318266723622425}{Bv}      & \BARdefault{636.0}{2.23}{12.59186034633817}{Bv}          & \BARdefault{235.2}{1.10}{5.889500504049451}{Bv}       & \BARdefault{33.9}{1.02}{5.354897369287726}{Bv}       \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize V100} & \BARreference{197.5}{1.00}{5.285936066969417}{Y}      & \BARreference{233.1}{1.00}{5.451366263509908}{Y}         & \BARreference{555.9}{1.00}{6.32061312855457}{Y}       & \BARreference{92.1}{1.00}{4.52246908433353}{Y}       & \BARreference{45.4}{1.00}{3.816088415905452}{Y}          & \BARreference{45.8}{1.00}{3.823453397811408}{Y}      & \BARreference{285.6}{1.00}{5.654538387490948}{Y}         & \BARreference{214.4}{1.00}{5.36782936697844}{Y}       & \BARreference{33.3}{1.00}{5.258935123867509}{Y}      \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 3080} & \BARpattern{145.1}{0.73}{3.8814933012206123}{Bv!60}   & \BARpattern{146.9}{0.63}{3.435856228627084}{Bv!60}       & \BARpattern{641.3}{1.15}{7.291371549839283}{Bv!60}    & \BARpattern{94.1}{1.02}{4.623142532302552}{Bv!60}    & \BARpattern{38.6}{0.85}{3.2452160735822675}{Bv!60}       & \BARpattern{61.4}{1.34}{5.13048529670323}{Bv!60}     & \BARpattern{529.4}{1.85}{10.48224497924457}{Bv!60}       & \BARpattern{244.1}{1.14}{6.111642645204826}{Bv!60}    & \BARpattern{44.9}{1.35}{7.08837949839249}{Bv!60}     \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 8000} & \BARpattern{83.5}{0.42}{2.2337814185841833}{gray!20}  & \BARpattern{145.9}{0.63}{3.4126326426965803}{gray!20}    & \BARpattern{332.5}{0.60}{3.7802886921611982}{gray!20} & \BARpattern{61.3}{0.67}{3.011878291562434}{gray!20}  & \BARpattern{26.2}{0.58}{2.201974760917085}{gray!20}      & \BARpattern{41.4}{0.91}{3.4627309669899793}{gray!20} & \BARpattern{173.0}{0.61}{3.4256383578045013}{gray!20}    & \BARpattern{159.3}{0.74}{3.98812027409279}{gray!20}   & \BARpattern{27.6}{0.83}{4.3624955249724895}{gray!20} \\[-1.0ex]
    \raisebox{1.5pt}{\scriptsize 5000} & \BARpattern{70.3}{0.36}{1.8824115491574087}{gray!10}  & \BARpattern{97.9}{0.42}{2.2908153465739565}{gray!10}     & \BARpattern{244.4}{0.44}{2.778768289746811}{gray!10}  & \BARpattern{53.4}{0.58}{2.6211586833107114}{gray!10} & \BARpattern{21.2}{0.47}{1.7776130911623143}{gray!10}     & \BARpattern{31.9}{0.70}{2.6650271064039828}{gray!10} & \BARpattern{220.2}{0.77}{4.358990425844327}{gray!10}     & \BARpattern{121.7}{0.57}{3.0459559540601724}{gray!10} & \BARpattern{22.7}{0.68}{3.578613394326972}{gray!10}  \\[-1.0ex]
    \\[-1ex]
\end{tabular}

==> eval/eval_header.tex <==
\input{../setting/font_libertinus}
\usepackage[scaled=.9]{newtxtt}

\newcommand{\BOLD}{\fontfamily{ugq}\selectfont}
% \newcommand{\EVALTITLE}[1]{\color{B}\bfseries\sffamily#1\hspace{0.6em}}
\newcommand{\EVALTITLE}[1]{\color{black}\BOLD#1}

\input{../setting/module_color}
\input{../setting/module_tikz}

%% 
%% https://alexwlchan.net/2017/10/latex-underlines/
\usepackage{contour}
\usepackage{ulem}

\renewcommand{\ULdepth}{2.2pt}
\contourlength{0.3pt}

\newcommand{\UnderLine}[1]{%
    \renewcommand{\ULthickness}{2.0pt}
    {\color{Y}\uline{\phantom{#1}}}%
    \llap{\contour{white}{#1}}%
}



\newcommand{\TIME}[4]{%% #1 val, #2 ratio, #3 platform, #4 color
    \begin{tikzpicture}
        \draw[anchor=east, draw=none, fill=none] (0,-.2) rectangle ++(-.01, .4);
        \begin{scope}%[yshift=0.1cm]
            \node[anchor=east, inner sep=0] at (0, 0) {\tiny#1};
            \node[anchor=west, inner sep=0] at (0, 0) {};
        \end{scope}
    \end{tikzpicture}%
}


\newcommand{\BARbase}[6]{%% #1 val, #2 ratio, #3 draw-len #4 color, #5 pattern setting, #6 draw border
    \hspace{.5em}%
    \begin{tikzpicture}
        \pgfmathtruncatemacro{\perct}{#2*100}%
        \draw[anchor=east, draw=#6, fill=#4] (-4.3em,-0.12) rectangle ++(-{#3}*\SCALE, 0.25);
        \draw[anchor=east, draw=none, #5] (-4.3em,-0.12) rectangle ++(-{#3}*\SCALE, 0.25);
        \begin{scope}%[yshift=0.1cm]
            \node[anchor=east, inner sep=0] at (-0.05, 0) {%
                \makebox[2.2em][r]{\scriptsize\raisebox{0pt}{{\color{gray}\perct\%}}%
                    \makebox[3.6em][r]{\small{#1}}%
                }%
            };
        \end{scope}
    \end{tikzpicture}%
}

\newcommand{\BARdefault}[4]{%% #1 val, #2 ratio, #3 draw-len #4 color
    \BARbase{#1}{#2}{#3}{#4}{}{none}%
}

\newcommand{\BARreference}[4]{%% #1 val, #2 ratio, #3 draw-len #4 color
    \BARbase{#1}{#2}{#3}{gray!40}{}{none}%
}

\newcommand{\BARaux}[4]{%% #1 val, #2 ratio, #3 draw-len #4 color
    \BARbase{#1}{#2}{#3}{none}{}{black}%
}


\newcommand{\BARpattern}[4]{%% #1 val, #2 ratio, #3 draw-len #4 color
    \BARbase{#1}{#2}{#3}{#4}{pattern=crosshatch dots, pattern color=gray}{none}%
}






==> figure/header.tex <==
\input{../setting/module_color}
\input{../setting/module_math}
\input{../setting/module_tikz}
\input{../setting/module_tabular}
\input{../setting/font_libertinus}
\usepackage[scaled=.96]{newtxtt}



\arrayrulecolor{gray!40}

==> listing/alg_sz-cx.tex <==
\small\ttfamily
\begin{algorithmic}[1] % The number tells where the line numbering should start
\For{$d\in D$ cascadingly}
    \Comment{{\color{B}\fontfamily{ugq}\selectfont compression}}
    \State $p^\circ \gets\ell(d_\textsc{\scshape sr})$, $e^\circ \gets p^\circ\! - d$
    \If{$e^\circ/eb < $ \textsc{cap (in-cap)} }   \Comment{quantization}
        \State $q^{\circ\phantom{\star}}    \gets$ \textsc{integerize}$(e^\circ/(2\!\times\!eb))$
        \State $d^{\circ\star}              \gets  p^\circ + 2\cdot e^\circ_\text{D}\cdot eb$
        \State $q^{\circ\phantom{\star}}    \gets  |d^{\circ\star}\! - d| < eb$ \AlgoMark{?} $q^\circ$ \AlgoMark{:} 0 \Comment{recheck}
    \Else
        \State $q^\circ \gets 0$ and append verbatim $(x\equiv d)$ to outlier
    \EndIf
    \State $d\gets$ $d^{\circ\star}$ or $x$ accordingly
    \Comment{incurs \textsc{\bfseries raw}}
\EndFor
\Statex
\For{$d^\bullet\in D^\bullet$ cascadingly}
\Comment{{\color{B}\fontfamily{ugq}\selectfont decompression}}
    \State $p^\bullet \gets  \ell(d^\bullet_\text{\scshape sr})$
    \State $d^\bullet \gets$ \textsc{in-cap} \AlgoMark{?} $ p^\bullet + 2\cdot e^\circ_\text{D}\cdot eb$ \AlgoMark{:} verbatim $x$
\EndFor
\end{algorithmic}

==> listing/tab_datasets.tex <==
\begin{tabular}{@{} l r r r @{}}
\tableTitleFormat datasets
    & \tableTitleFormat type
    & \datumSize{\footnotesize datum size}{\tableTitleFormat dimensions}
    & \dataTableBase{\#fields}{\tableTitleFormat example(s)}{r}
\\ [.5ex]
\toprule
\datasetName{cosmology}{HACC}
    % & 6
    & \ttfamily fp32
    & \datumSize{1,071.75 MB}{280,953,867}
    %, or 
    % \datumSize{}{1,073,726,487}
    & \datasetField{6}{x, vx}
\\
\datasetName{climate}{CESM-ATM}
    % & 79 
    & \ttfamily fp32
    & \datumSize{24.72 MB}{1,800$\times$3,600} 
    & \datasetField{79}{CLDHGH, CLDLOW}
\\
\datasetName{climate}{Hurricane}
    % & 20 
    & \ttfamily fp32
    & \datumSize{95.37 MB}{100$\times$500$\times$500} 
    & \datasetField{20}{CLOUDf48, Uf48}
\\
\datasetName{cosmology}{Nyx}
    % & 6 
    & \ttfamily fp32
    & \datumSize{512.00 MB}{512$\times$512$\times$512}
    & \datasetField{6}{baryon\_density}
\\
\datasetName{quantum}{QMCPACK}
    % & 1
    & \ttfamily fp32
    & \datumSize{601.52 MB}{288$\times$115$\times$69$\times$69}
    & \datasetField{2 formats}{einspline}
\\
\bottomrule
\end{tabular}

==> listing/tab_eval.tex <==
% \newcommand{\TabUnitStyle}{\scshape\bfseries\sffamily\color{gray}}
\begin{tabular}{@{} l@{} r@{} rrr rr rr @{}}   
&
& \grandTableTitle{r}{predict. (p)}{\bfseries + quant. (q)}
& 
& \grandTableTitle{r}{huffman}{}
& 
& \grandTableTitle{r}{kernel}{compression}
& \grandTableTitle{r}{gpu-to-cpu}{\footnotesize \textsc{valrel}@10\textsuperscript{-4}}
& \grandTableTitle{r}{overall}{compression}
   \\ 
\toprule    
&       
& \TabUnitStyle mb/s
&       
& \TabUnitStyle mb/s
&       
& 
&       
& \TabUnitStyle mb/s
\\
\textsc{\sffamily CPU-SZ} 
& \textsc{\sffamily hacc}  
& 137.7 
&       
& 328.6 
&       
& - %94.1 
& -     
& 94.1 \\
          
& \textsc{\sffamily cesm-atm} 
& 105.0
&       
& 459.1 
&       
& - %85.5 
& -     
& 85.5 \\
          
& \textsc{\sffamily hurricane} 
& 93.8 
&       
& 504.0
&       
& - %78.5 
& -     
& 78.5 \\
          
& \textsc{\sffamily nyx}   
& 98.5 
&       
& 648.7 
&       
& - %84.7 
& -     
& 84.7 \\
          
& \textsc{\sffamily qmcpack} 
& 97.5 
&       
& 396.2 
&       
& - %80.8 
& -     
& 80.8 \\
\midrule
&
& 
& {\color{black}\scshape histogram}
& {\color{black}\scshape codebook}
& {\color{black}\scshape coding}
& 
& 
& 
\\[-.4ex]
&       
& \TabUnitStyle gb/s
& \TabUnitStyle gb/s
& \TabUnitStyle ms
& \TabUnitStyle gb/s
& \TabUnitStyle gb/s
& \TabUnitStyle gb/s
& \TabUnitStyle gb/s
\\
\textsc{\sffamily\scshape cuSZ} 
& \textsc{\sffamily hacc}  
& 207.7
& 602.8 
& 5.16
& 54.1
& 40.0
& 53.2	%% comm: CR=4.954
& 22.8 
\\          
& \textsc{\sffamily cesm-atm} 
& 252.1
& 345.3 
& 4.33
& 57.2
& 41.1 
& 81.9	%% comm: CR=10.378
& 27.4 
\\          
& \textsc{\sffamily hurricane} 
& 175.8
& 418.0
& 4.81 
& 55.2 
& 38.2 
& 40.8	%% comm: CR=927
& 19.7	
\\          
& \textsc{\sffamily nyx}   
& 200.2
& 427.6 
& 3.84
& 58.8
& 41.1 
& 134.1	%% comm: CR=12.84
& 31.6 
\\
& \textsc{\sffamily qmcpack} 
& 189.6
& 346.1 
& 4.09
& 61.0
& 40.7 
& 99.2	%% comm: CR=9.47
& 28.9 
\\
\midrule
{\sffamily cuZFP} 
& \textsc{\sffamily hacc}  
& -     
& -     
& -     
& -     
& -     
& -     
& - \\
          
& \textsc{\sffamily cesm-atm} 
& -     
& -     
& -     
& -     
& 47.6 		%% bitrate=12   
& 27.7      %% CR=2.67
& 17.5 \\
          
& \textsc{\sffamily hurricane} 
& -     
& -     
& -     
& -     
& 83.7 		%% bitrate=12
& 27.7 		%% CR=32/12=2.67
& 20.8 \\
          
& \textsc{\sffamily nyx}   
& -     
& -     
& -     
& -     
& 71.3		%% bitrate=6
& 56.3		%% CR=32/6=5.33, alternatively, 1/4.8 the NYX cuSZ
& 31.7 \\
          
& \textsc{\sffamily qmcpack} 
& -     
& -     
& -     
& -     
& 72.6		%% bitrate=8, psnr @83.98
& 42.5		%% CR=4     
& 26.8 \\
\bottomrule

\end{tabular}
\quad
\begin{tabular}{@{} r rr @{}}   
  \grandTableTitle{r}{huffman}{\color{black}\scshape decoding}
& \grandTableTitle{r}{reversed}{\bfseries\scshape(p+q)}
& \grandTableTitle{r}{kernel}{\scshape\hskip -1em decompression}
   \\ 
\toprule
  \TabUnitStyle mb/s
& \TabUnitStyle mb/s
& \TabUnitStyle mb/s
\\
	196.0
&	659.3
& 	151.1
\\
	502.2
&	451.9
&	237.9
\\
	524.5
&	306.8
&	185.0
\\
	670.4
&	300.5
&	201.8
\\
	660.3
&	313.4
&	211.1
\\
\midrule
\scshape canonical
\\[-.4ex]
  \textsc{dec.\hspace{.66em}\TabUnitStyle gb/s}
& \TabUnitStyle gb/s
& \TabUnitStyle gb/s
\\
  35.0	& 16.8	& 11.4	\\
  41.6	& 58.5	& 24.3	\\
  34.2	& 43.9	& 19.2	\\
  52.4	& 29.7	& 19.0	\\
  40.3	& 22.4	& 14.4	\\
\midrule
  - & - & - 	\\ 
  - & - & 113.1 	\\ 
  - & - & 102.2 \\ 
  -	& - & 103.1	\\ 
  -	& - & 115.5	\\ 
\bottomrule

\end{tabular}




==> listing/tab_eval_k.tex <==
\begin{tabular}{@{} l@{} r@{} rrr rr rr @{}}   
&
& \grandTableTitle{r}{\bfseries predict. (p)}{\bfseries\scshape + quant. (q)}
& %\grandTableTitle{r}{\bfseries huffman}{\color{gray}histogram}
& \grandTableTitle{r}{\bfseries huffman}{}%\grandTableTitle{r}{\bfseries huffman}{\color{gray}codebook}
& %\grandTableTitle{r}{\bfseries huffman}{\color{gray}encoding}
& \grandTableTitle{r}{\bfseries kernel}{\scshape compression}
& \grandTableTitle{r}{\bfseries gpu-to-cpu}{\footnotesize \textsc{valrel}@10\textsuperscript{-4}}
& \grandTableTitle{r}{\bfseries overall}{compression}
   \\ 
\toprule    
&       
& \textsc{\bfseries\sffamily\color{gray}mb/s}
&       
& \textsc{\bfseries\sffamily\color{gray}mb/s}
&       
& 
&       
& \textsc{\bfseries\sffamily\color{gray}mb/s}
\\
\textsc{\sffamily CPU-SZ} 
& \textsc{\sffamily hacc}  
& 137.7 
&       
& 328.6 
&       
& - %94.1 
& -     
& 94.1 \\
          
& \textsc{\sffamily cesm-atm} 
& 105.0
&       
& 459.1 
&       
& - %85.5 
& -     
& 85.5 \\
          
& \textsc{\sffamily hurricane} 
& 93.8 
&       
& 504.0
&       
& - %78.5 
& -     
& 78.5 \\
          
& \textsc{\sffamily nyx}   
& 98.5 
&       
& 648.7 
&       
& - %84.7 
& -     
& 84.7 \\
          
& \textsc{\sffamily qmcpack} 
& 97.5 
&       
& 396.2 
&       
& - %80.8 
& -     
& 80.8 \\
\midrule
&
& %\grandTableTitle{r}{\bfseries prediction+}{\bfseries\scshape quantization}
& {\color{black}\scshape histogram}
& {\color{black}\scshape codebook}
& {\color{black}\scshape coding}
& %\grandTableTitle{r}{\bfseries kernel}{compression}
& %\grandTableTitle{r}{\bfseries gpu-to-cpu}{\footnotesize \textsc{valrel}@10\textsuperscript{-4}}
& %\grandTableTitle{r}{\bfseries overall}{compression}
\\[-.4ex]
&       
& \textsc{\bfseries\sffamily\color{gray}gb/s}
& \textsc{\bfseries\sffamily\color{gray}gb/s}
& \textsc{\bfseries\sffamily\color{gray}ms}    
& \textsc{\bfseries\sffamily\color{gray}gb/s}
& \textsc{\bfseries\sffamily\color{gray}gb/s}
& \textsc{\bfseries\sffamily\color{gray}gb/s}
& \textsc{\bfseries\sffamily\color{gray}gb/s}
\\
\textsc{\sffamily\scshape cuSZ} 
& \textsc{\sffamily hacc}  
& 207.7
& 602.8 
& 5.16
& 54.1
& 40.0
& 53.2	%% comm: CR=4.954
& 22.8 
\\          
& \textsc{\sffamily cesm-atm} 
& 252.1
& 345.3 
& 4.33
& 57.2
& 41.1 
& 81.9	%% comm: CR=10.378
& 27.4 
\\          
& \textsc{\sffamily hurricane} 
& 175.8
& 418.0
& 4.81 
& 55.2 
& 38.2 
& 40.8	%% comm: CR=927
& 19.7	
\\          
& \textsc{\sffamily nyx}   
& 200.2
& 427.6 
& 3.84
& 58.8
& 41.1 
& 134.1	%% comm: CR=12.84
& 31.6 
\\
& \textsc{\sffamily qmcpack} 
& 189.6
& 346.1 
& 4.09
& 61.0
& 40.7 
& 99.2	%% comm: CR=9.47
& 28.9 
\\
\midrule
{\sffamily cuZFP} 
& \textsc{\sffamily hacc}  
& -     
& -     
& -     
& -     
& -     
& -     
& - \\
          
& \textsc{\sffamily cesm-atm} 
& -     
& -     
& -     
& -     
& 47.6 		%% bitrate=12   
& 27.7      %% CR=2.67
& 17.5 \\
          
& \textsc{\sffamily hurricane} 
& -     
& -     
& -     
& -     
& 83.7 		%% bitrate=12
& 27.7 		%% CR=32/12=2.67
& 20.8 \\
          
& \textsc{\sffamily nyx}   
& -     
& -     
& -     
& -     
& 71.3		%% bitrate=6
& 56.3		%% CR=32/6=5.33, alternatively, 1/4.8 the NYX cuSZ
& 31.7 \\
          
& \textsc{\sffamily qmcpack} 
& -     
& -     
& -     
& -     
& 72.6		%% bitrate=8, psnr @83.98
& 42.5		%% CR=4     
& 26.8 \\
\bottomrule

\end{tabular}
\quad
\begin{tabular}{@{} r rr @{}}   
  \grandTableTitle{r}{\bfseries huffman}{\color{black}\scshape decoding}
& \grandTableTitle{r}{\bfseries reversed}{\bfseries\scshape (p+q)}
& \grandTableTitle{r}{\bfseries kernel}{\scshape\hskip -1em decompression}
   \\ 
\toprule
  \textsc{\bfseries\sffamily\color{gray}mb/s}
& \textsc{\bfseries\sffamily\color{gray}mb/s}
& \textsc{\bfseries\sffamily\color{gray}mb/s}
\\
	196.0
&	659.3
& 	151.1
\\
	502.2
&	451.9
&	237.9
\\
	524.5
&	306.8
&	185.0
\\
	670.4
&	300.5
&	201.8
\\
	660.3
&	313.4
&	211.1
\\
\midrule
\scshape canonical
\\[-.4ex]
  \textsc{dec.\hspace{.66em}\bfseries\sffamily\color{gray}gb/s}
& \textsc{\bfseries\sffamily\color{gray}gb/s} 
& \textsc{\bfseries\sffamily\color{gray}gb/s}
\\
  35.0	& 16.8	& 11.4	\\
  41.6	& 58.5	& 24.3	\\
  34.2	& 43.9	& 19.2	\\
  52.4	& 29.7	& 19.0	\\
  40.3	& 22.4	& 14.4	\\
\midrule
  - & - & - 	\\ 
  - & - & 113.1 	\\ 
  - & - & 102.2 \\ 
  -	& - & 103.1	\\ 
  -	& - & 115.5	\\ 
\bottomrule

\end{tabular}




==> listing/tab_nearzero.tex <==
{\setlength{\tabcolsep}{4pt}  
\renewcommand{\arraystretch}{1.2}
% \newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
% \newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = `bottom' strut

\begin{tabular}{@{}|lllllll|l|@{}}
% \toprule
\multicolumn{8}{l@{}}{\bfseries CLOUDf48} \\
\hline
min & 1\%   & 25\%  & 50\%  & 75\%  & 99\%  & max & range \\
0.00e+0 & 0.00e+0 & 0.00e+0 & 0.00e+0 & 0.00e+0 & 2.53e-4 & 2.05e-3 & 2.05e-3 \\
\hline
\multicolumn{8}{@{}|l| @{}}{\makebox[6.5em][l]{$\phantom{\frac{1}{10}}eb=$2.05e-7}\quad 89.20\% in $[-eb, eb]$, \hspace{2.63em}and 89.20\% in $[\text{min}, \text{min} + eb]$} \\
\multicolumn{8}{@{}|l| @{}}{\makebox[6.5em][l]{$\frac{1}{10}eb=$2.05e-8}\quad 88.50\% in $[-\frac{1}{10}eb, \frac{1}{10}eb]$, and 88.50\% in $[\text{min}, \text{min} + \frac{1}{10}eb]$} 
\\[.4ex]
\hline
% \midrule
\multicolumn{8}{l@{}}{\bfseries QSNOWf48} \\
\hline
min & 1\%   & 25\%  & 50\%  & 75\%  & 99\%  & max & range \\
0.00e+0 & 0.00e+0 & 1.11e-10 & 1.96e-9 & 6.34e-9 & 6.01e-5 & 8.56e-4 & 8.56e-4 \\
\hline
\multicolumn{8}{@{}|l| @{}}{\makebox[6.5em][l]{$\phantom{\frac{1}{10}}eb=$8.56e-8}\quad 88.90\% in $[-eb, eb]$, \hspace{2.63em}and 88.90\% in $[\text{min}, \text{min} + eb]$} \\
\multicolumn{8}{@{}|l| @{}}{\makebox[6.5em][l]{$\frac{1}{10}eb=$8.56e-9}\quad 80.90\% in $[-\frac{1}{10}eb, \frac{1}{10}eb]$, and 80.90\% in $[\text{min}, \text{min} + eb]$} 
\\[.4ex]
\hline
% \midrule
\multicolumn{8}{l@{}}{\bfseries baryon density} \\
\hline
min & 1\%   & 25\%  & 50\%  & 75\%  & 99\%  & max & range \\
5.80e-2 & 1.37e-1 & 3.22e-1 & 5.06e-1 & 8.75e-1 & 7.42e+0 & 1.16e+5 & 1.16e+5 \\
\hline
\multicolumn{8}{@{}|l| @{}}{\makebox[6.5em][l]{$\phantom{\frac{1}{10}}eb=$1.16e+1}\quad 99.50\% in $[-eb, eb]$, \hspace{2.63em}and 99.50\% in $[\text{min}, \text{min} + eb]$} \\
\multicolumn{8}{@{}|l| @{}}{\makebox[6.5em][l]{$\frac{1}{10}eb=$1.16e+0}\quad 83.30\% in $[-\frac{1}{10}eb, \frac{1}{10}eb]$, and 84.40\% in $[\text{min}, \text{min} + \frac{1}{10}eb]$} 
\\[.4ex]
\hline
% \bottomrule
\end{tabular}%
}


%
%\begin{tabular}{@{} r rrr @{}}
%\multicolumn{1}{c}{} 
%& \textbf{CLOUDf48} 
%& \textbf{QSNOWf48}
%& \textbf{baryon density} 
%\\[.1ex]
%\toprule
%eb   & 2.05e-7 & 8.56e-8 & 1.16E+01 \\
%\midrule
%min  & 0.0e+0 & 0.0e+0 & 5.8e-2 \\
%1\%  & 0.0e+0 & 0.0e+0 & 1.4e-1 \\
%25\% & 0.0e+0 & 1.1e-1\makebox[0pt][l]{0} & 3.2e-1 \\
%50\% & 0.0e+0 & 2.0e-9 & 5.1e-1 \\
%75\% & 0.0e+0 & 6.3e-9 & 8.8e-1 \\
%99\% & 2.5e-4 & 6.0e-5 & 7.4e+0 \\
%max  & 2.1e-3 & 8.6e-4 & 1.2e+5 \\
%\midrule
%range & 2.1e-3 & 8.6e-4 & 1.2e+5 \\
%\midrule
%in $[-eb,eb]$ & 89.2\% & 88.9\% & 99.5\% \\
%in $[\text{min}, \text{min} + eb]$ & 89.2\% & 88.9\% & 99.5\% \\
%in $[-\frac{1}{10}eb, \frac{1}{10}eb]$ & 88.5\% & 80.9\% & 83.3\% \\
%in $[\text{min}, \frac{1}{10}eb]$ & 88.5\% & 80.9\% & 84.4\% \\
%\bottomrule
%\end{tabular}%



==> listing/tab_par.tex <==

\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{}r|c|c|c|c|@{}}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \multicolumn{1}{r}{\color{B}\BOLD compression}
                                     & \TabTitle{sequential\ }
                                     & \TabTitle{\begin{minipage}{4em}coarse-\\[-.5ex]grained\end{minipage}}
                                     & \TabTitle{\begin{minipage}{4em}fine-\\[-.5ex]grained\end{minipage}}
                                     & \TabTitle{atomic}
    \\
    \cline{2-5}
    \textsc{dual-quant} construction &                                      &      & \YES &      \\
    \cline{2-5}
    histogram                        &                                      &      & \YES & \YES \\
    \cline{2-5}
    build Huffman tree               & \YES                                 &      &      &      \\
    \cline{2-5}
    canonize codebook                & \YES                                 &      & \YES & \YES \\
    \cline{2-5}
    Huffman encode (fix-length)      &                                      &      & \YES &      \\
    \cline{2-5}
    deflate	(to sparse format)        &                                      & \YES &      &      \\
    \cline{2-5}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \multicolumn{1}{r}{\color{B}\BOLD decompression}                                             \\
    \cline{2-5}
    Huffman decode                   &                                      & \YES &      &      \\
    \cline{2-5}
    reconstruction                   &                                      & \YES &      &      \\
    \cline{2-5}
\end{tabular}

==> listing/tab_perf-encode-deflate.tex <==
\sffamily
\begin{tabular}{@{}l@{}r@{}rrrrr@{}}
% & \doubleLineTableHead{r}{\tiny\color{GRAY}1 GB}{hacc}
&
& \doubleLineTableHead{r@{}}{\scriptsize\color{GRAY}1071 MB}{hacc}
& \doubleLineTableHead{r@{}}{\scriptsize\color{GRAY}25 MB}{cesm-atm}
& \doubleLineTableHead{r@{}}{\scriptsize\color{GRAY}95 MB}{hurricane}
& \doubleLineTableHead{r@{}}{\scriptsize\color{GRAY}512 MB}{nyx} 
& \doubleLineTableHead{r@{}}{\scriptsize\color{GRAY}602 MB}{qmcpack}
\\
% & \singleLineTableHeadFormat hacc
% & \singleLineTableHeadFormat cesm-atm
% & \singleLineTableHeadFormat hurricane
% & \singleLineTableHeadFormat Nyx 
% & \singleLineTableHeadFormat qmcpack
% \\
\toprule
   enc.64 
&   \scriptsize\color{GRAY} $\mu$s
&   \scriptsize\color{GRAY} 4,274.3 
&   \scriptsize\color{GRAY} 97.1
&   \scriptsize\color{GRAY} 385.8 
&   \scriptsize\color{GRAY} 2,044.7 
&   \scriptsize\color{GRAY} 2,401.4 
\\[-.5ex]
&   \scriptsize GB/s
&   250.9
&   255.1
&   251.7
&   251.1
&   251.1
\\
\midrule
   enc.32
&  \scriptsize\color{GRAY}   $\mu$s
&  \scriptsize\color{GRAY}   2,839.3
&  \scriptsize\color{GRAY}   64.1
&  \scriptsize\color{GRAY}   255.8 
&  \scriptsize\color{GRAY}   1,358.6   
&  \scriptsize\color{GRAY}   1,595.6
\\[-.5ex]
&   \scriptsize GB/s
&	377.7
&	386.6
&	379.6
&	377.9
&	377.9 
\\
\bottomrule
\end{tabular}


% \begin{tabular}{@{}l@{}r@{}rrrrr@{}}
% % & \doubleLineTableHead{r}{\tiny\color{GRAY}1 GB}{hacc}
% &
% & \doubleLineTableHead{r@{}}{\scriptsize\color{GRAY}1071 MB}{hacc}
% & \doubleLineTableHead{r@{}}{\scriptsize\color{GRAY}25 MB}{cesm-atm}
% & \doubleLineTableHead{r@{}}{\scriptsize\color{GRAY}95 MB}{hurricane}
% & \doubleLineTableHead{r@{}}{\scriptsize\color{GRAY}512 MB}{nyx} 
% & \doubleLineTableHead{r@{}}{\scriptsize\color{GRAY}602 MB}{qmcpack}
% \\
% % & \singleLineTableHeadFormat hacc
% % & \singleLineTableHeadFormat cesm-atm
% % & \singleLineTableHeadFormat hurricane
% % & \singleLineTableHeadFormat Nyx 
% % & \singleLineTableHeadFormat qmcpack
% % \\
% \toprule
%  encoding 
% &\scriptsize\color{GRAY} $\mu$s
% &  \scriptsize\color{GRAY} 4,274.3 
% &  \scriptsize\color{GRAY} \bfseries\color{BLUE} 97.1
% &  \scriptsize\color{GRAY} 385.8 
% &  \scriptsize\color{GRAY} 2,044.7 
% &  \scriptsize\color{GRAY} 2,401.4 
% \\[-.5ex]
% &\scriptsize GB/s
% &   250.6
% &   \bfseries\color{BLUE} 248.6
% &   259.3
% &   262.6
% &   262.7
% \\
%  deflating 
% &\scriptsize\color{GRAY} ms 
% &  \scriptsize\color{GRAY} 101.04 
% &  \scriptsize\color{GRAY} \bfseries\color{BLUE} 0.40 
% &  \scriptsize\color{GRAY} 7.12
% &  \scriptsize\color{GRAY} 54.27
% &  \scriptsize\color{GRAY} 47.51
% \\[-.5ex]
% &\scriptsize GB/s
% & 11.1  
% & \bfseries\color{BLUE} 60.3
% & 14.0
% & 9.9
% & 13.3
% \\
%  total 
% &\scriptsize\color{GRAY} ms 
% & \scriptsize\color{GRAY} 105.31  
% & \scriptsize\color{GRAY} \bfseries\color{BLUE} 0.50 
% & \scriptsize\color{GRAY} 7.51
% & \scriptsize\color{GRAY} 56.31
% & \scriptsize\color{GRAY} 49.91
% \\[-.5ex]
% &\scriptsize GB/s
% & 10.6  
% & \bfseries\color{BLUE} 48.3  
% & 13.3
% & 9.5 
% & 12.7
% \\
% \bottomrule
% 32-bit	\\
% \toprule
%  encoding 
% &\scriptsize\color{GRAY} $\mu$s
% &  \scriptsize\color{GRAY}
% &  \scriptsize\color{GRAY} \bfseries\color{BLUE} 67.7
% &  \scriptsize\color{GRAY}  
% &  \scriptsize\color{GRAY}  
% &  \scriptsize\color{GRAY}  
% \\[-.5ex]
% &\scriptsize GB/s
% &   
% &   \bfseries\color{BLUE} 356.6
% &   
% &   
% &   
% \\
%  deflating 
% &\scriptsize\color{GRAY} ms 
% &  \scriptsize\color{GRAY} 
% &  \scriptsize\color{GRAY} \bfseries\color{BLUE} 0.33
% &  \scriptsize\color{GRAY}
% &  \scriptsize\color{GRAY} 
% &  \scriptsize\color{GRAY} 
% \\[-.5ex]
% &\scriptsize GB/s
% & 
% & \bfseries\color{BLUE} 72.3
% & 
% & 
% & 
% \\
%  total 
% &\scriptsize\color{GRAY} ms 
% & \scriptsize\color{GRAY} 
% & \scriptsize\color{GRAY} \bfseries\color{BLUE} 0.40
% & \scriptsize\color{GRAY} 
% & \scriptsize\color{GRAY} 
% & \scriptsize\color{GRAY} 
% \\[-.5ex]
% &\scriptsize GB/s
% & 
% & \bfseries\color{BLUE} 60.3
% & 
% & 
% & 
% 	\\
% \bottomrule
% \end{tabular}

==> listing/tab_psnr-similarity.tex <==
\sffamily
\begin{tabular}{@{}lrrlrr@{}}
\singleLineTableHeadFormat field     & \textsc{\sffamily\bfseries SZ-1.4} & \textsc{\sffamily\bfseries cuSZ} &   \singleLineTableHeadFormat field    & \textsc{\sffamily\bfseries SZ-1.4} & \textsc{\sffamily\bfseries cuSZ} \\
\toprule
%%%%%%%
    \texttt{CLOUDf48} & 84.99 & 94.18 & \texttt{QSNOWf48} & 84.31 & 93.36 \\
    \texttt{CLOUDf48.log10} & 84.51 & 87.17 & \texttt{QSNOWf48.log10} & 84.87 & 84.93 \\
    \texttt{Pf48} & 84.79 & 84.79 & \texttt{QVAPORf48} & 84.79 & 84.80 \\
    \texttt{PRECIPf48} & 85.35 & 92.86 & \texttt{TCf48} & 84.79 & 84.79 \\
    \texttt{PRECIPf48.log10} & 84.82 & 84.77 & \texttt{Uf48} & 84.79 & 84.79 \\
    \texttt{QCLOUDf48} & 85.03 & 98.91 & \texttt{Vf48} & 84.79 & 84.79 \\
    \texttt{QCLOUDf48.log10} & 85.22 & 95.21 & \texttt{Wf48} & 84.79 & 84.79 \\
\addlinespace[-0.7ex]
\cmidrule(l){4-6}
\addlinespace[-0.8ex]
\texttt{QGRAUPf48} & 88.21 & 97.02 & \texttt{baryon\_density} & 89.71 & 98.25 \\
    \texttt{QGRAUPf48.log10} & 84.90 & 84.82 & \texttt{dark\_matter\_density} & 86.57 & 87.77 \\
    \texttt{QICEf48} & 84.61 & 95.51 & \texttt{temperature} & 84.77 & 84.77 \\
    \texttt{QICEf48.log10} & 85.56 & 85.77 & \texttt{velocity\_x} & 84.77 & 84.77 \\
    \texttt{QRAINf48} & 85.36 & 97.37 & \texttt{velocity\_y} & 84.77 & 84.77 \\
    \texttt{QRAINf48.log10} & 84.93 & 84.56 & \texttt{velocity\_z} & 84.77 & 84.77 \\
\midrule
    \sffamily Hurricane avg. & 85.01 & 86.96 & \sffamily Nyx avg. & 85.58 & 85.98 \\
    \bottomrule
\end{tabular}%

==> listing/tab_rate-discortion.tex <==
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}r|rrr|rrr|@{}}
    \multicolumn{1}{c}{}
&   bitrate &   CR  & \multicolumn{1}{c}{PSNR}
&   bitrate &   CR  & \multicolumn{1}{c}{PSNR}
\\
\cline{2-4}\cline{5-7}
\scshape cesm-atm  &   3.08 bits   &   10.4    &   85.3 dB     &   12 bits &   2.7    &   88.7 dB
\\
\scshape hurricane  &   3.45 bits   &   9.3    &   87.0 dB     &   12 bits &   2.7    &   81.9 dB
\\
\scshape nyx        &   2.49 bits   &   12.8   &   86.0 dB     &    6 bits &   5.3    &   85.1 dB
\\
\scshape qmcpack    &   3.38 bits   &   9.5    &   85.0 dB     &    8 bits &   4.0    &   84.0 dB
\\[.5ex]
\cline{2-4}\cline{5-7}
    \multicolumn{1}{c}{}
&   \multicolumn{3}{c}{\bfseries\textsc{cuSZ}}
&   \multicolumn{3}{c}{\bfseries cuZFP}
\\
\end{tabular}

==> listing/tab_tree-time.tex <==
\sffamily
\begin{tabular}{@{}l 
    % *{7}{r} 
    *{4}{>{\raggedleft\arraybackslash}p{2.0em}} 
    *{3}{>{\raggedleft\arraybackslash}p{2.2em}} 
@{}}
    \singleLineTableHeadFormat\#quant. 
    & \singleLineTableHeadFormat 128 
    & \singleLineTableHeadFormat 256
    & \singleLineTableHeadFormat 512
    & \singleLineTableHeadFormat 1024
    & \singleLineTableHeadFormat 2048 
    & \singleLineTableHeadFormat 4096 
    & \singleLineTableHeadFormat 8192 
    \\
\toprule
\sffamily build tree	
    &	{0.48}
    &	0.77
    &   1.80
%    &   3.367
	&	{2.13}
    &   6.46
    &   12.68
    &   25.06
\\
\sffamily get codebook
    &   {0.20}
    &   1.14
    &   2.36
%    &   3.987
	&	{2.69}
    &   7.09
    &   14.43
    &   25.65
\\
\sffamily total
    &   {0.68}
    &   2.16
    &   4.16
%    &   7.354
	&	{4.81}
    &   13.55
    &   27.10
    &   50.71
\\
\bottomrule
\end{tabular}

==> listing/tab_tune.tex <==
% \begin{table*}[ht]
\footnotesize\sffamily
\newcommand{\CTITLE}{\scshape\sffamily\bfseries\small}
\newcommand{\HLNUM}[1]{\bfseries #1}

\resizebox{\linewidth}{!}{%
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}l@{}}
\\
\sffamily\scshape\bfseries chunk \\
\sffamily\scshape\bfseries size  \\
\toprule
2$^\text{6}$  \\
2$^\text{7}$  \\
2$^\text{8}$  \\
2$^\text{9}$  \\
2$^\text{10}$ \\
2$^\text{11}$ \\
2$^\text{12}$ \\
2$^\text{13}$ \\
2$^\text{14}$ \\
2$^\text{15}$ \\
2$^\text{16}$ \\
\bottomrule
\end{tabular}
\enspace

\begin{tabular}{@{}rrr@{}}
\multicolumn{3}{@{}l}{\CTITLE hacc}
\\
\multicolumn{3}{@{}l}{\scshape\sffamily\color{gray} 1071.8 mb\quad 280,953,867 \sf f32} 
\\
  \scshape\sffamily\#thread 
& \scshape\sffamily deflate 
& \scshape\sffamily inflate
\\
\toprule
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
    1.4e5 & 4.6   & 2.8 \\
    6.9e4 & 5.1   & 5.1 \\
    3.4e4 & 13.6  & 12.1 \\
    \HLNUM{1.7e4} & \HLNUM{63.1} & \HLNUM{35.0} \\
    8.6e3 & 65.8  & 28.1 \\
    4.3e3 & 45.9  & 14.3 \\
\bottomrule
\end{tabular}
\enspace

\begin{tabular}{@{}rrr@{}}
\multicolumn{3}{@{}l}{\CTITLE cesm}
\\
\multicolumn{3}{@{}l}{\scshape\sffamily\color{gray} 24.7 mb\quad 6,480,000 \sf f32} 
\\
  \scshape\sffamily\#thread 
& \scshape\sffamily deflate 
& \scshape\sffamily inflate
\\
\toprule
    {1.0e5} & 11.3 & 25.0 \\
    {5.1e4} & 15.5 & 37.8 \\
     \HLNUM{2.5e4}  &  \HLNUM{67.1}   &  \HLNUM{41.6}   \\
    {1.3e4} & 55.6 & 30.7 \\
    {6.3e3} & 48.2 & 19.6 \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
    \bottomrule
\end{tabular}
\enspace

\begin{tabular}{@{}rrr@{}}
\multicolumn{3}{@{}l}{\CTITLE hurricane}
\\
\multicolumn{3}{@{}l}{\scshape\sffamily\color{gray} 95.4 mb\quad 25,000,000 \sf f32} 
\\
  \scshape\sffamily\#thread 
& \scshape\sffamily deflate 
& \scshape\sffamily inflate
\\
\toprule
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
    {9.8e4} & 5.1 & 11.0 \\
    {4.9e4} & 10.2 & 9.4 \\
     \HLNUM{2.4e4}  &  \HLNUM{64.6}   &  \HLNUM{34.2}   \\
    {1.2e4} & 57.3 & 27.7 \\
    {6.1e3} & 50.7 & 17.8 \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
    \bottomrule
\end{tabular}
\enspace

\begin{tabular}{@{}rrr@{}}
\multicolumn{3}{@{}l}{\CTITLE nyx} 
\\
\multicolumn{3}{@{}l}{\scshape\sffamily\color{gray} 512 mb\quad 134,217,728 \sf f32} 
\\
  \scshape\sffamily\#thread 
& \scshape\sffamily deflate 
& \scshape\sffamily inflate
\\
\toprule
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
    {1.3e5} & 4.7 & 5.9 \\
    {6.6e4} & 5.7 & 6.3 \\
    {3.3e4} & 25.1 & 16.1 \\
     \HLNUM{1.6e4}  &  \HLNUM{69.7}   &  \HLNUM{52.4}   \\
    {8.2e3} & 72.4 & 42.6 \\
    {4.1e3} & 50.0 & 23.1 \\
       $.$    &    $.$    &    $.$     \\
    \bottomrule
\end{tabular}
\enspace

\begin{tabular}{@{}rrr@{}}
\multicolumn{3}{@{}l}{\CTITLE qmcpack}
\\
\multicolumn{3}{@{}l}{\scshape\sffamily\color{gray} 601.5 mb\quad 157,684,320 \sf f32}
\\
  \scshape\sffamily\#thread 
& \scshape\sffamily deflate 
& \scshape\sffamily inflate
\\
\toprule
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
       $.$    &    $.$    &    $.$     \\
    {1.5e5} & 4.7 & 5.1 \\
    {7.7e4} & 5.2 & 6.2 \\
    {3.8e4} & 12.9 & 11.1 \\
     \HLNUM{1.9e4}  &  \HLNUM{72.7}   & \HLNUM{40.3} \\
    {9.6e3} & 75.9 & 29.0 \\
    {4.8e3} & 56.0 & 16.1 \\
       $.$    &    $.$    &    $.$     \\
    \bottomrule
\end{tabular}%
}


==> setting/_metadata.tex <==

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
% \begin{CCSXML}
% <ccs2012>
%  <concept>
%   <concept_id>10010520.10010553.10010562</concept_id>
%   <concept_desc>Computer systems organization~Embedded systems</concept_desc>
%   <concept_significance>500</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010575.10010755</concept_id>
%   <concept_desc>Computer systems organization~Redundancy</concept_desc>
%   <concept_significance>300</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010553.10010554</concept_id>
%   <concept_desc>Computer systems organization~Robotics</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10003033.10003083.10003095</concept_id>
%   <concept_desc>Networks~Network reliability</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Computer systems organization~Embedded systems}
% \ccsdesc[300]{Computer systems organization~Redundancy}
% \ccsdesc{Computer systems organization~Robotics}
% \ccsdesc[100]{Networks~Network reliability}

%\begin{CCSXML}
%<ccs2012>
%   <concept>
%       <concept_id>10003752.10003809.10010170.10010174</concept_id>
%       <concept_desc>Theory of computation~Massively parallel algorithms</concept_desc>
%       <concept_significance>500</concept_significance>
%       </concept>
% </ccs2012>
%\end{CCSXML}

%\ccsdesc[500]{Theory of computation~Massively parallel algorithms}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.

%\keywords{GPU, Massively Parallel, Lossy Compression}

%% A "teaser" image appears between the author and affiliation
%% information and the body of the document, and typically spans the
%% page.
% \begin{teaserfigure}
%   \includegraphics[width=\textwidth]{sampleteaser}
%   \caption{Seattle Mariners at Spring Training, 2010.}
%   \Description{Enjoying the baseball game from the third-base
%   seats. Ichiro Suzuki preparing to bat.}
%   \label{fig:teaser}
% \end{teaserfigure}

==> setting/author_acm.tex <==
\newcommand{\wsu}{Washington State University}
\newcommand{\ua}{The University of Alabama}
\newcommand{\ucr}{University of California, Riverside}
\newcommand{\clemson}{Clemson University}
\newcommand{\anl}{Argonne National Laboratory}
\newcommand{\ornl}{Oak Ridge National Laboratory}

\newcommand{\AFFIL}[3]{%
    \affiliation{%
        \institution{\small #1}
        % \city{#2}\state{#3}\country{USA}
    }
    }

\newcommand{\WSU}{\AFFIL{\wsu}{Pullman}{WA}}
\newcommand{\UA}{\AFFIL{\ua}{Tuscaloosa}{AL}}
\newcommand{\UCR}{\AFFIL{\ucr}{Riverside}{CA}}
\newcommand{\ANL}{\AFFIL{\anl}{Lemont}{IL}}
\newcommand{\ORNL}{\AFFIL{\ornl}{Oak Ridge}{TN}}
\newcommand{\CLEMSON}{\AFFIL{\clemson}{Clemson}{SC}}

% \let\oldauthor\author
% \renewcommand{\author}[1]{{\large\oldauthor{#1}}}

\author{Jiannan Tian}{\WSU}
\email{jiannan.tian@wsu.edu}

\author{Sheng Di}{\ANL}
\email{sdi1@anl.gov}

\author{Kai Zhao}{\UCR}
\email{kzhao016@ucr.edu}

\author{Cody Rivera}{\UA}
\email{cjrivera1@crimson.ua.edu}

\author{Megan Hickman Fulp}{\CLEMSON}
\email{mlhickm@g.clemson.edu}

\author{Robert Underwood}{\CLEMSON}
\email{robertu@g.clemson.edu}

\author{Sian Jin}{\WSU}
\email{sian.jin@wsu.edu}

\author{Xin Liang}{\ORNL}
\email{liangx@ornl.gov}

\author{Jon Calhoun}{\CLEMSON}
\email{jonccal@clemson.edu}

\author{Dingwen Tao}
\authornote{Corresponding author: Dingwen Tao (\url{dingwen.tao@wsu.edu}), School of EECS, Washington State University, Pullman, WA 99164, USA.}
{\WSU}
\email{dingwen.tao@wsu.edu}

\author{Franck Cappello}{\ANL}
\email{cappello@mcs.anl.gov}


% \author{%
%     Jiannan Tian,$^{\star}$ 
%     Sheng Di,$^{\S}$ 
%     Kai Zhao,$^{\dagger}$ 
%     Cody Rivera,$^\ddagger$
%     Megan Hickman Fulp,$^\xi$ 
%     Robert Underwood,$^\xi$
%     Sian Jin,$^\star$
%     Xin Liang,$^\dagger$
%     Jon Calhoun,$^\xi$
%     Dingwen Tao,$^\star$ and
%     Franck Cappello$^\S$
%   }
% \authornote{Corresponding author: Dingwen Tao (\url{dingwen.tao@wsu.edu}), School of EECS, Washington State University, Pullman, WA 99164, USA.}

% \newcommand{\AUTH}[4]{
%     \begin{tabular}{@{}c@{}} 
%     \large #1\makebox[0.2em][l]{$^{#4}$}    \\[-.3ex]
%     \normalsize #3          \\[-.5ex]
%     \sffamily\small #2
%     \end{tabular}%
%     }

% \affiliation{
% \centering
% \begin{tabular}{@{}cccc@{}}
% \AUTH{Jiannan Tian}{jiannan.tian@wsu.edu}{\wsu}{}
% &   \AUTH{Sheng Di}{sdi1@anl.gov}{\anl}{}
% &   \AUTH{Kai Zhao}{kzhao016@ucr.edu}{\makebox[1.6in][c]{\ucr}}{}
% &   \AUTH{Cody Rivera}{cjrivera1@crimson.ua.edu}{\ua}{}
% \\[3ex]
% \AUTH{Megan Hickman Fulp}{mlhickm@g.clemson.edu}{\clemson}{}
% &   \AUTH{Robert Underwood}{robertu@g.clemson.edu}{\clemson}{}
% &   \AUTH{Sian Jin}{sian.jin@wsu.edu}{\wsu}{\star}
% &   \AUTH{Xin Liang}{liangx@ornl.gov}{\makebox[1.6in][c]{\ornl}}{}
% \end{tabular}
% \\[.5ex]
% \begin{tabular}{ccc}
% \AUTH{Jon Calhoun}{jonccal@clemson.edu}{\makebox[1.6in][c]{\clemson}}{}
% &   \AUTH{Dingwen Tao}{dingwen.tao@wsu.edu}{\wsu}{}\authornote{Corresponding author: Dingwen Tao (\url{dingwen.tao@wsu.edu}), School of EECS, Washington State University, Pullman, WA 99164, USA.}
% &   \AUTH{Franck Cappello}{cappello@mcs.anl.gov}{\anl}{}
% \end{tabular}
% }


\renewcommand{\shortauthors}{Tian et~al.}

==> setting/author_ieee_journal.tex <==
\author{
        Jiannan Tian,
        Sheng Di, %~\IEEEmembership{Senior Member,~IEEE,} 
        Cody Rivera,
        Xiaodong Yu,
        Griffin Dube,
        Kai Zhao,
        Megan Hickman Fulp,\\
        Robert Underwood,
        Sian Jin,
        Jon Calhoun,
        Xin Liang,
        Dingwen Tao,
        and Franck Cappello%,~\IEEEmembership{Fellow,~IEEE}% <-this % stops a space
        
\IEEEcompsocitemizethanks{
\IEEEcompsocthanksitem J. Tian, S. Jin, and D. Tao are with the School of Electrical Engineering \& Computer Science, Washington State University, Pullman, WA 99164.\protect
%E-mail: \{jiannan.tian, sian.jin, dingwen.tao\}@wsu.edu

\IEEEcompsocthanksitem X. Yu is with the Data Science and Learning Division, S. Di and F. Cappello are with the Mathematics and Computer Science Division, Argonne National Laboratory, Lemont, IL 60439.\protect
%E-mail: xyu@anl.gov
%E-mail: sdi1@anl.gov, cappello@mcs.anl.gov

\IEEEcompsocthanksitem C. Rivera is with the Department of Computer Science, The University of Alabama,
Tuscaloosa, AL 35405.\protect
%E-mail: cjrivera1@crimson.ua.edu

\IEEEcompsocthanksitem G. Dube, M. Flup, R. Underwood, and J. Calhoun are with the College of Engineering, Clemson University, Clemson, SC 29634.\protect
%E-mail: \{mlhickm, robertu\}@g.clemson.edu, jonccal@clemson.edu 

\IEEEcompsocthanksitem K. Zhao is with the Department of Computer Science \& Engineering, University of California, Riverside, Riverside, CA 92521.\protect
%E-mail: kzhao016@ucr.edu

\IEEEcompsocthanksitem X. Liang is with the Department of Computer Science, Missouri University of Science and Technology, Rolla, MO 65409.\protect
%E-mail: xliang@mst.edu

\IEEEcompsocthanksitem D. Tao (dingwen.tao@wsu.edu) is the corresponding author.
\protect
}

% <-this % stops an unwanted space
% \thanks{
% Manuscript received April 19, 2005; revised August 26, 2015.}
}


==> setting/font_libertinus.tex <==
\usepackage[sb]{libertinus}
\usepackage{libertinust1math}

==> setting/module_codelisting.tex <==
% \usepackage{listings}						% code listing
% \lstset{
%     basicstyle=\ttfamily\small,     %%% string settings
%     stringstyle=\color{R},
%     keywordstyle=\color{B2}\bfseries,
%     commentstyle=\color{gray},
%     tabsize=2,
%     breaklines=true,
%     showstringspaces=false,
%     showspaces=false,
%     %backgroundcolor=\color{gray!4}, 
%     xleftmargin=6pt,
%     framexleftmargin=6pt,
%     framesep=0pt,
%     numberstyle=\bfseries\ttfamily\scriptsize\color{R},
%     numbers=left, % {none, left, right}; position of line number
%     numbersep=6pt, % how far the line-numbers are from the code
%     stepnumber=1, % the step between two line-numbers. If it's 1, each line will be numbered
%     escapeinside={Ω}{≈}
% }

==> table/header.tex <==
\input{../setting/module_color}
\input{../setting/module_tikz}
\input{../setting/module_math}
\input{../setting/module_tabular}
\input{../setting/module_styles}
\input{../setting/module_text_macros}

%\input{../setting/font_libertinus}
\usepackage[scaled=.96]{newtxtt}


==> table/intro-par-cites.tex <==
            \renewcommand{\arraystretch}{1.43}
            \newcommand{\GoodCitingCusz}{\textcolor{B}{\cite{cusz2020}}}
            \newcommand{\SoSoCitingCusz}{\textcolor{gray}{\cite{cusz2020}}}
            \scriptsize
            \begin{tabular}{@{}l@{}}
                {\GoodCitingCusz}                                  \\    %% dual-quant
                {\GoodCitingCusz} \cite{cuSPARSE98:online} {[}+{]} \\    %% cusparse
                \cite{GmezLuna2012AnOA}                            \\    %% histogram
                \cite{ostadzadeh2007practical}                     \\
                \SoSoCitingCusz                                    \\ %% huffman encoding
                \SoSoCitingCusz                                    \\ %% deflate
                \\
                \cite{weissenberger2018massively}                  \\ %% massive huffman decoding
                \cite{cuSPARSE98:online}                           \\ %% scatter
                {[}+{]}                                            \\
            \end{tabular}

==> table/tab-demo-int-fp.tex <==
\begin{tabular}{@{}rlr@{}}
        \texttt{int(511)}   &
        % view in bytes       & 
        \texttt{00000000 00000000 00000001 11111111} \\
    \texttt{float(511)} & 
    % view in bytes    & 
    \texttt{01000011 11111111 10000000 00000000} \\[1ex]
                        % & view of IEEE-754 & \texttt{0 10000111 11111111000000000000000} \\[1ex]
      \texttt{int(512)} & 
    %   view in bytes    &
      \texttt{00000000 00000000 00000010 00000000} \\
    \texttt{float(512)} & 
    % view in bytes    & 
    \texttt{01000100 00000000 00000000 00000000} \\
                        % & view of IEEE-754 & \texttt{0 10001000 00000000000000000000000}
    \end{tabular}
